Nucleon resonances and transition form factors

This is a contribution to the review 50 Years of Quantum Chromodynamics edited by F. Gross and E. Klempt, to be published in Journal EPJC. This contribution reviews the nucleon resonance transition form factors determined from meson electro-production experiments at electron accelerator facilities, i.e. this contribution focuses on space-like transition form factors and amplitudes. Comparisons are made when available to LQCD and to approaches with traceable links to strong QCD and to advanced quark model calculations

==> authors.tex <==
\centerline {\huge  Volker D. Burkert} \\  \
\bigskip

\centerline {\Large Thomas Jefferson National Accelerator Facility} \\ 

\centerline {\Large 12000 Jefferson Avenue, 
Newport News, Virginia, 23606, USA}
